Synthesizing Programmatic Reinforcement Learning Policies with Large Language Model Guided Search

Programmatic reinforcement learning (PRL) has been explored for representing policies through programs as a means to achieve interpretability and generalization. Despite promising outcomes, current state-of-the-art PRL methods are hindered by sample inefficiency, necessitating tens of millions of program-environment interactions. To tackle this challenge, we introduce a novel LLM-guided search framework (LLM-GS). Our key insight is to leverage the programming expertise and common sense reasoning of LLMs to enhance the efficiency of assumption-free, random-guessing search methods. We address the challenge of LLMs' inability to generate precise and grammatically correct programs in domain-specific languages (DSLs) by proposing a Pythonic-DSL strategy - an LLM is instructed to initially generate Python codes and then convert them into DSL programs. To further optimize the LLM-generated programs, we develop a search algorithm named Scheduled Hill Climbing, designed to efficiently explore the programmatic search space to improve the programs consistently. Experimental results in the Karel domain demonstrate our LLM-GS framework's superior effectiveness and efficiency. Extensive ablation studies further verify the critical role of our Pythonic-DSL strategy and Scheduled Hill Climbing algorithm. Moreover, we conduct experiments with two novel tasks, showing that LLM-GS enables users without programming skills and knowledge of the domain or DSL to describe the tasks in natural language to obtain performant programs.

==> figure/dsl.tex <==
\begin{wrapfigure}[15]{R}{0.45\textwidth}
\centering
\vspace{-0.5cm}
\begin{mdframed}[font=\scriptsize]
\vspace{-0.35cm}
{
    \begin{align*}
    \text{Program}\ \rho &\coloneqq \text{DEF}\  \text{run}\ \text{m}(\ s\ \text{m})\\
    \text{Repetition} \ n &\coloneqq \text{0..19}\\
    \text{Perception} \ h & \coloneqq \text{frontIsClear} \ | \ \text{leftIsClear} \ | \  \text{rightIsClear} \ | \ \\ 
    & \text{markersPresent} \ | \ \text{noMarkersPresent} \\
    \text{Condition} \ b &\coloneqq \text{perception h} \ | \ \text{not} \ \text{perception h} \\
    \text{Action} \ a &\coloneqq \text{move} \ | \ \text{turnLeft}
    \ | \ \text{turnRight} \ | \ \\
    & \text{putMarker} \ | \ \text{pickMarker} \\
    \text{Statement}\ s &\coloneqq \text{WHILE}\ \text{c}(\ b\ \text{c})\ \text{w}(\ s\ \text{w}) \ | \ s_1 s_2 \ | \ a \ | \\ 
    & \ \text{REPEAT}\ \text{R=}n\ \text{r}(\ s\ \text{r}) \ | \ \text{IF}\ \text{c}(\ b\ \text{c})\ \text{i}(\ s\ \text{i}) \ | \\ 
    & \ \text{IFELSE}\ \text{c}(\ b\ \text{c})\ \text{i}(\ s_1\ \text{i}) \  \text{ELSE}\ \text{e}(\ s_2\ \text{e}) \\
    \end{align*}
\vspace{-0.85cm}
}
\end{mdframed}
    \vspace{-0.2cm}
    \caption[]{
        \small
        The domain-specific language (DSL) for the Karel domain, features an agent that can navigate through a grid world and interact with objects.
        \yenchun{Figure is obtained from \citet{liu2023hprl}.}
    }
    \label{fig:dsl}
\end{wrapfigure}

==> figure/dsl_and_doorkey.tex <==
\begin{figure}[t]
\centering
    \scalebox{0.95}{
    \begin{subfigure}[b]{0.3\textwidth}
    \begin{mdframed}[font=\scriptsize]
    \vspace{-0.35cm}
    {
    \begin{align*}
    \text{Program}\ \rho &\coloneqq \text{DEF}\  \text{run}\ \text{m}(\ s\ \text{m})\\
    \text{Repetition} \ n &\coloneqq \text{0..19}\\

    \text{Perception} \ h & \coloneqq \text{frontIsClear} \ | \ \text{leftIsClear} \ | \  \text{rightIsClear} \ | \ \\ 
    & \text{markersPresent} \ | \ \text{noMarkersPresent} \\
    \text{Condition} \ b &\coloneqq \text{perception h} \ | \ \text{not} \ \text{perception h} \\
    \text{Action} \ a &\coloneqq \text{move} \ | \ \text{turnLeft}
    \ | \ \text{turnRight} \ | \ \\
    & \text{putMarker} \ | \ \text{pickMarker} \\
    \text{Statement}\ s &\coloneqq \text{WHILE}\ \text{c}(\ b\ \text{c})\ \text{w}(\ s\ \text{w}) \ | \ s_1 s_2 \ | \ a \ | \\ 
    & \ \text{REPEAT}\ \text{R=}n\ \text{r}(\ s\ \text{r}) \ | \ \text{IF}\ \text{c}(\ b\ \text{c})\ \text{i}(\ s\ \text{i}) \ | \\ 
    & \ \text{IFELSE}\ \text{c}(\ b\ \text{c})\ \text{i}(\ s_1\ \text{i}) \  \text{ELSE}\ \text{e}(\ s_2\ \text{e}) \\
    \end{align*}
    \vspace{-0.85cm}
    }
    \end{mdframed}
    \end{subfigure}
    }
    \hfill
    \begin{subfigure}[b]{0.54\textwidth}
         \centering
        \includegraphics[width=\linewidth]{figure/Doorkey.pdf}
     \end{subfigure}

    \caption{\textbf{The Karel Domain Specific Language~(DSL) grammar~(left).} Figure is obtained from HPRL~\citep{liu2023hprl}. Actions, perceptions, and~basic control flows can be used to write DSL programs to solve Karel tasks. \textbf{An example Karel task -- \doorkey~(right).} The agent need to first find the key, and then navigate to the goal in another room. This task has been found to pose significant challenges to previous PRL methods. \yenchun{need fact check}
    \sun{let's make the doorkey fig smaller and the dsl larger. the fontsize is imbalance}
    \yenchun{One student need to volunteer to combine / polish this figure. Key: 1. roughly align height. 2. text font size should be similar @Chan-Hung please assign some one.}
    }\yu{chengwei will do the work}
    \label{fig:prelim}
\end{figure}



==> figure/init_necessity_ablation.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/init_necessity_ablation/doorkey.png}
        \caption{\doorkey}
        \label{fig:init_necessity_ablation_doorkey}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/init_necessity_ablation/cleanhouse.png}
        \caption{\cleanhouse}
        \label{fig:init_necessity_ablation_cleanhouse}
    \end{subfigure}
    \caption{
        \textbf{Comparing initializations.} 
        We compare initializing the search population using LLM-generated programs or randomly sampled programs.
        The results show that starting from LLM-generated programs significantly improves efficiency, highlighting the effectiveness of our proposed framework.
    }
    \label{fig:init_necessity_ablation}
\end{figure}

==> figure/main_results_backup.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{\doorkey}
        \label{fig:sub1}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f2}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f3}
        \label{fig:sub3}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{ f1}
        \label{fig:sub1}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f2}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f3}
        \label{fig:sub3}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{ f1}
        \label{fig:sub1}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f2}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f3}
        \label{fig:sub3}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.8\textwidth]{figure/main_results/Snake_log.png}
        \caption{f3}
        \label{fig:sub3}
    \end{subfigure}
    \caption{Figure}
    \label{fig:big}
    \caption{
    \yenchun{Please don't worry about space for now and put figures that are easy to read. Expand each subfig to a full figure. We can polish together later. Also, you can put the table latext snippet to the table folder and use the input command  (it's easier for moving paper around)}\yu{Shao-Hua asked me to show this kind of preview figure for him, so I will first leave it like this.}
    }
\end{figure}

==> figure/new_environment_results.tex <==
\begin{wrapfigure}[15]{r}{0.49\textwidth}
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figure/minigrid_results/lavagap.png}
            \caption{\lavagap}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figure/minigrid_results/putnear.png}
            \caption{\putnear}
        \end{subfigure}
        \vspace{-0.6cm}
        \caption{
            \textbf{Performance of \lavagap{} \& \putnear{}.}
            By transforming all components of the prompt from the Karel domain to the Minigrid version, our proposed method surpasses the best-performing baseline HC, highlighting the extensibility of LLM-GS. 
        }
        \label{fig:new environment results}
    \end{minipage}
\end{wrapfigure}


==> figure/new_tasks_results.tex <==
\begin{wrapfigure}[15]{r}{0.49\textwidth}
  \centering
  \begin{minipage}{0.49\textwidth}
    \centering
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figure/rebuttal/pathfollow.png}
            \caption{\pathfollow}
        \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figure/rebuttal/wallavoider.png}
            \caption{\wallavoider}
            \label{fig:init_necessity_ablation_cleanhouse}
        \end{subfigure}
        \vspace{-0.6cm}
        \caption{
            \textbf{Performance of \pathfollow{} \& \wallavoider{}.} 
            With only changing the task description, our proposed method surpasses the best-performing baseline HC, highlighting the extensibility of LLM-GS. 
        }
        \label{fig:new tasks results}
    \end{minipage}
\end{wrapfigure}


==> table/llm_prompt_full.tex <==

\begin{table}[t]
\centering
\caption{
\textbf{Environment and DSL awareness of the LLM.}
We utilize the system prompt to teach LLM the underlying physics of the target environment, alongside the detailed specifications of the domain specific language~(DSL). For the Karel environment, we decribe the \emph{environment physics} in natural language. The DSL is specified via a \emph{constrained} version of the Python programming language with pre-define functions.
The \emph{DSL perceptions} allow the agent to observe the environment, and the \emph{DSL actions} allow the agent to interact with the environment.
}
\label{tab:llm_prompt_full}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{1.0\columnwidth}{L p{0.8\columnwidth}}
\toprule
\textbf{Knowledge} & \textbf{Prompt Text} \\
 \midrule
Environment Knowledge & You're currently navigating within a Karel environment, which is essentially a grid world. In this context, a ``world'' is referred to as a ``map.'' Within this map, there's an entity known as the ``agent,'' capable of movement, changing direction, as well as picking up and placing markers on the map. Additionally, there are obstacles called ``walls'' that impede the agent's progress; whenever the agent encounters a wall, it turns around. Furthermore, there are pre-existing ``markers'' scattered throughout the map at the beginning, though the agent has the ability to both pickup and place these markers as needed. \\
\midrule
 
\multirow{5}{}{DSL Perceptions} & \texttt{frontIsClear()}: Returns \texttt{True} if there is no wall in front of the agent.\\
& \texttt{leftIsClear():} Returns \texttt{True} if there is no wall on the agent's left.\\
& \texttt{rightIsClear()}: Returns \texttt{True} if there is no wall on the agent's right.\\
& \texttt{markersPresent()}: Returns \texttt{True} if there exist markers on the current cell.\\
& \texttt{noMarkersPresent()}: Returns \texttt{True} if there is no marker on the current cell. \\

\midrule
\multirow{5}{}{DSL Actions} & \texttt{move()}: Asks the agent to move forward one cell. The agent will instead turn left twice if a wall is blocking its way.\\
& \texttt{turnLeft()}: Asks the agent to rotate 90 degrees counter-clockwise.\\
& \texttt{turnRight()}: Asks the agent to rotate 90 degrees clockwise.\\
 & \texttt{pickMarker()}: Asks the agent to pick up one marker from the current cell.\\
 & \texttt{putMarker()}: Asks the agent to put down one marker on the current cell. \\
 
\midrule
\multirow{4}{}{Language Constraints} & - do not define other functions besides \texttt{run()}\\
& - do not call other functions\\
& - do not define variables\\
& - do not use \texttt{True}, \texttt{False}, \texttt{break}, \texttt{continue}, \texttt{return}, \texttt{==}, \texttt{!=}, \texttt{elif}, \texttt{or}, \texttt{and} \\

\midrule
Output Instruction & Your objective is to generate the appropriate Python program based on a given task name and description. This Python program will encompass actions enabling the agent to engage with the environment, alongside perceptions facilitating the agent's recognition of the environment's dynamics. \\

\bottomrule
\end{tabularx}
\end{table}


==> table/llm_prompt_specific_full.tex <==
\begin{table}[t]


\centering
\caption{
\textbf{Activate the LLM's task awareness.}
To bridge the domain gap between the target task and the LLM's knowledge, we carefully curate the prompt to include only reasonable knowledge. One need to be cautious to not leak any task specific programming skill. We detail the full prompt for \doorkey here as an example. Given the task name, map description, initial position, task goal, and task reward, the LLM is encouraged to solve the specified task with its learned common sense.
\yenchun{saving space: maybe we only need one of goal / reward?}
}
\label{tab:llm_prompt_specific}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{1.0\columnwidth}{L p{0.79\textwidth}}
\toprule
\textbf{Knowledge} & \textbf{Prompt Text} \\
 \midrule
Task Name & \small \doorkey \\
\midrule
Map Description &  \small The map is a $8 \times 8$ grid surrounded by walls that is vertically split into two chambers. The left chamber is $6 \times 3$ grid and the right chamber is $6 \times 2$ grid. There is a marker placed randomly on the left chamber as a key, and another marker placed randomly on the right chamber as a goal. \\
\midrule
Initial Position &  \small The agent starts on a random cell on the left chamber facing east. \\


\midrule
Task Goal & \small The goal of the agent is to pick up a marker on the left chamber, which opens a door connecting both chambers. Allow the agent to reach and put a marker on the goal marker. \\
\midrule
Task Reward & \small Picking up the first marker yields a $0.5$ reward, and putting a marker on the goal marker yields an additional $0.5$. \\

\bottomrule
\end{tabularx}
\end{table}



==> table/llm_revised_ablation.tex <==

\begin{table}[t]
\centering
\caption{
\textbf{LLM Revised}
\sun{maybe get rid of ours and just emphasize it in text}
}
\label{table:llm_revised}
\scalebox{0.75}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{3}{*}{\bf Task}
    & \multirow{2}{*}{\bf Before}
    & \multicolumn{2}{c}{\multirow{2}{*}{\bf Regenerate}}
    & \multicolumn{2}{c}{\bf Regenerate} 
    & \multicolumn{2}{c}{\bf Agent} 
    & \multicolumn{2}{c}{\bf Agent and Program} 
    \\
    &
    &
    &
    & \multicolumn{2}{c}{\bf with reward} 
    & \multicolumn{2}{c}{\bf execution trace} 
    & \multicolumn{2}{c}{\bf execution trace.}
    \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
    & Return
    & Return & Cost
    & Return & Cost
    & Return & Cost
    & Return & Cost
    \\
    \midrule
    \cleanhouse & 0.21$\pm$0.05 & 0.22$\pm$0.03 & \$1.77 & 0.27$\pm$0.11 & \$2.85 & 0.99$\pm$0.03 & \$4.17 & \textbf{0.99$\pm$0.02} & \$4.31\\\
    \doorkey & 0.61$\pm$0.15 & 0.70$\pm$0.12 & \$1.89 & 0.76$\pm$0.13 & \$3.06 & 0.73$\pm$0.11 & \$4.27 & \textbf{0.76$\pm$0.06} & \$4.45\\\
    \seeder & 0.67$\pm$0.10 & 0.75$\pm$0.15 & \$2.00 & \textbf{0.84$\pm$0.10} & \$3.24 & 0.83$\pm$0.15 & \$4.40 & 0.78$\pm$0.16 & \$4.60\\
        
    \bottomrule
    \end{tabular}
}
\end{table}
